Binary Optimization via Mathematical Programming with Equilibrium Constraints

Binary optimization is a central problem in mathematical optimization and its applications are abundant. To solve this problem, we propose a new class of continuous optimization techniques which is based on Mathematical Programming with Equilibrium Constraints (MPECs). We first reformulate the binary program as an equivalent augmented biconvex optimization problem with a bilinear equality constraint, then we propose two penalization/regularization methods (exact penalty and alternating direction) to solve it. The resulting algorithms seek desirable solutions to the original problem via solving a sequence of linear programming convex relaxation subproblems. In addition, we prove that both the penalty function and augmented Lagrangian function, induced by adding the complementarity constraint to the objectives, are exact, i.e., they have the same local and global minima with those of the original binary program when the penalty parameter is over some threshold. The convergence of both algorithms can be guaranteed, since they essentially reduce to block coordinate descent in the literature. Finally, we demonstrate the effectiveness and versatility of our methods on several important problems, including graph bisection, constrained image segmentation, dense subgraph discovery, modularity clustering and Markov random fields. Extensive experiments show that our methods outperform existing popular techniques, such as iterative hard thresholding, linear programming relaxation and semidefinite programming relaxation.

==> allfigures.tex <==
\clearpage


\begin{figure*}[!t]
\subfigure[cat image] {\includegraphics[width=0.3\textwidth]{./fig/cat.eps}}
\subfigure[by unary] {\includegraphics[width=0.3\textwidth]{./fig/cat_init.eps}}
\subfigure[by padmm] {\includegraphics[width=0.3\textwidth]{./fig/cat_padm.eps}}
\\
\subfigure[by box] {\includegraphics[width=0.3\textwidth]{./fig/cat_box.eps}}
\subfigure[by sa] {\includegraphics[width=0.3\textwidth]{./fig/cat_sa.eps}}
\subfigure[by icm] {\includegraphics[width=0.3\textwidth]{./fig/cat_icm.eps}}
\\
\subfigure[by crf] {\includegraphics[width=0.3\textwidth]{./fig/cat_crf.eps}}
\subfigure[by alpha] {\includegraphics[width=0.3\textwidth]{./fig/cat_gcAlpha.eps}}
\subfigure[by alphe-beta] {\includegraphics[width=0.3\textwidth]{./fig/cat_gcAlphaBeta.eps}}
\vspace{-5pt} \centering
\caption{Image Segmentation Result on Cat Image} \label{fig:exp:gamma}
\end{figure*}


\begin{figure*}[!t]
\subfigure[cat image] {\includegraphics[width=0.3\textwidth]{./fig/flower.eps}}
\subfigure[by unary] {\includegraphics[width=0.3\textwidth]{./fig/flower_init.eps}}
\subfigure[by padmm] {\includegraphics[width=0.3\textwidth]{./fig/flower_padm.eps}}
\\
\subfigure[by box] {\includegraphics[width=0.3\textwidth]{./fig/flower_box.eps}}
\subfigure[by sa] {\includegraphics[width=0.3\textwidth]{./fig/flower_sa.eps}}
\subfigure[by icm] {\includegraphics[width=0.3\textwidth]{./fig/flower_icm.eps}}
\\
\subfigure[by crf] {\includegraphics[width=0.3\textwidth]{./fig/flower_crf.eps}}
\subfigure[by alpha] {\includegraphics[width=0.3\textwidth]{./fig/flower_gcAlpha.eps}}
\subfigure[by alphe-beta] {\includegraphics[width=0.3\textwidth]{./fig/flower_gcAlphaBeta.eps}}
\vspace{-5pt} \centering
\caption{Image Segmentation Result on Cat Image} \label{fig:exp:gamma}
\end{figure*}



\begin{figure*}[!t]
\subfigure[cat image] {\includegraphics[width=0.3\textwidth]{./fig/man.eps}}
\subfigure[by unary] {\includegraphics[width=0.3\textwidth]{./fig/man_init.eps}}
\subfigure[by padmm] {\includegraphics[width=0.3\textwidth]{./fig/man_padm.eps}}
\\
\subfigure[by box] {\includegraphics[width=0.3\textwidth]{./fig/man_box.eps}}
\subfigure[by sa] {\includegraphics[width=0.3\textwidth]{./fig/man_sa.eps}}
\subfigure[by icm] {\includegraphics[width=0.3\textwidth]{./fig/man_icm.eps}}
\\
\subfigure[by crf] {\includegraphics[width=0.3\textwidth]{./fig/man_crf.eps}}
\subfigure[by alpha] {\includegraphics[width=0.3\textwidth]{./fig/man_gcAlpha.eps}}
\subfigure[by alphe-beta] {\includegraphics[width=0.3\textwidth]{./fig/man_gcAlphaBeta.eps}}
\vspace{-5pt} \centering
\caption{Image Segmentation Result on Cat Image} \label{fig:exp:gamma}
\end{figure*}





